ZEN: Pre-training Chinese Text Encoder Enhanced by N-gram Representations

The pre-training of text encoders normally processes text as a sequence of tokens corresponding to small text units, such as word pieces in English and characters in Chinese. It omits information carried by larger text granularity, and thus the encoders cannot easily adapt to certain combinations of characters. This leads to a loss of important semantic information, which is especially problematic for Chinese because the language does not have explicit word boundaries. In this paper, we propose ZEN, a BERT-based Chinese (Z) text encoder Enhanced by N-gram representations, where different combinations of characters are considered during training. As a result, potential word or phase boundaries are explicitly pre-trained and fine-tuned with the character encoder (BERT). Therefore ZEN incorporates the comprehensive information of both the character sequence and words or phrases it contains. Experimental results illustrated the effectiveness of ZEN on a series of Chinese NLP tasks. We show that ZEN, using less resource than other published encoders, can achieve state-of-the-art performance on most tasks. Moreover, it is shown that reasonable performance can be obtained when ZEN is trained on a small corpus, which is important for applying pre-training techniques to scenarios with limited data. The code and pre-trained models of ZEN are available at https://github.com/sinovation/zen.

==> complexity.tex <==
\subsection{Training Complexities}
%5.1重写时空分析, 现在只有时间分析没有空间分析，别人用了多少显存  space memory
%看看别人有没有gpu性能换算 在文章里可以写一个，我们follow别人的时间分析做法

%

\begin{table}[t]
\begin{center}
\begin{sc}
\begin{small}
\arrayrulecolor{black}
\begin{tabular}{lrr} 
\arrayrulecolor{black}\toprule
Models  & Space & Time (size)\\ 
\midrule
BERT & 24.73 & 400 (1.3G)\\
\hline
BERT-wwm  & 24.73 & $\approx$1200 (1.3G)\\ 
ERNIE 1.0 & 24.73 & $\approx$3000 (10.7G)\\ 
% ERNIE 2.0 (B) &  & -\\ 
% ERNIE 2.0 (L) &  & -\\ 
\hline
ZEN (R) & 37.40 & 400 (1.3G)\\
ZEN (P) & 37.40 & 100 (1.3G)\\
\arrayrulecolor{black}\bottomrule
\end{tabular}
\end{small}
\vspace{-0.3cm}
\end{sc}
\end{center}
\caption{Comparison of ZEN against other pre-trained models. The total GPU memory (GB) used for pre-training and the estimated training time (hours) on a V100 GPU are reported.}
\label{complex}
\vspace{-1.0em}
\end{table}

To pre-train a text encoder, one often requires a huge amount of data and computation resources,
as indicated in existing studies \citep{devlin2018bert, sun2019ernie, sun2019ernie2}.  
%
Owing to the limitation of resources, a well-designed encoder is expected to train efficiently with fewer resources.
%As an aspect to illustrate
Therefore, we compare the complexities of ZEN and existing encoders
with respect to their space and time requirements in pre-training.
%
%ZEN can be trained with limited computational resources comparing to other Chinese encoders.
%To conduct the comparison, we roughly 
%
Consider that different models in previous studies are trained on different devices, e.g., BERT and BERT-wwm are trained on TPUs, it is hard to compare their complexities precisely.
Herein we apply NVidia Tesla V100 GPU as the standard and transfer the computation power of other devices into that equivalent to V100 GPUs, i.e., 
%The computational power of
a TPU is roughly estimated by 8 V100 GPUs.\footnote{\textcolor{cyan}{https://medium.com/bigdatarepublic/cost-comparison-of-deep-learning-hardware-google-tpuv2-vs-nvidia-tesla-v100-3c63fe56c20f}}
%
The results are shown in Table \ref{complex}.
We note that our ZEN model, which uses the same dataset as that of the original BERT, also has a similar time complexity as the original BERT, although extra space is required to accommodate n-gram encoding. On the other hand, other methods, trying to achieve higher accuracy, used significantly more resources.


